Words as Gatekeepers: Measuring Discipline-specific Terms and Meanings in Scholarly Publications

Scholarly text is often laden with jargon, or specialized language that can facilitate efficient in-group communication within fields but hinder understanding for out-groups. In this work, we develop and validate an interpretable approach for measuring scholarly jargon from text. Expanding the scope of prior work which focuses on word types, we use word sense induction to also identify words that are widespread but overloaded with different meanings across fields. We then estimate the prevalence of these discipline-specific words and senses across hundreds of subfields, and show that word senses provide a complementary, yet unique view of jargon alongside word types. We demonstrate the utility of our metrics for science of science and computational sociolinguistics by highlighting two key social implications. First, though most fields reduce their use of jargon when writing for general-purpose venues, and some fields (e.g., biological sciences) do so less than others. Second, the direction of correlation between jargon and citation rates varies among fields, but jargon is nearly always negatively correlated with interdisciplinary impact. Broadly, our findings suggest that though multidisciplinary venues intend to cater to more general audiences, some fields' writing norms may act as barriers rather than bridges, and thus impede the dispersion of scholarly ideas.

==> old_paragraphs.tex <==
The majority of past work on creating maps of science have leveraged citation information, such as co-citation and inter-citation frequencies \cite{boyack2005mapping,VANECK2014802,morris2008mapping,fortunato2018science}. Citation networks have also been used to create vector-space representations of journals \cite{peng2021neural} and uncover fields of science \cite{rosvall2008maps}. \citet{shahaf2012metro}, when motivating their decision to use citations rather than language to map science, claims that shared keywords such as \textit{probability}, \textit{cost}, and \textit{network} may overestimate the similarity of different research areas. Our present work lessens this alleged pitfall by not only looking at word types, but also their in-context uses. 

A smaller subset of research on science has used a language-focused perspective \citep[e.g.][]{yogatama-etal-2011-predicting,mckeown2016predicting,prabhakaran-etal-2016-predicting,vilhena2014finding}. Language differences often indicate different communities, such as factions of authors \cite{sim-etal-2012-discovering} and disciplinary approaches \cite{ngai2018discourse,west-portenoy-2016-delineating}. Language has also been used to measure the innovation of ideas and topics \cite{gerow2018measuring, hofstra2020diversity}. Most language-centered studies of science focus on words and phrases, though a few have examined word meaning or use, such as semantic progressiveness over time \cite{soni2021follow} and semantic uncertainty of words in ambiguous contexts \cite{mcmahan2018ambiguity}. Research on polysemy or homonymy in science is more prominent in education, with an emphasis on how to improve the teaching of overloaded terminology \cite{ryan1985language,cervetti2015factors}. 

Some maps of science have combined both citation information and language, such as keywords \cite{borner2012design}. As a notable example, \citet{vilhena2014finding} uses language to identify ``cultural holes'' in science, and they suggest that this provides a related, but distinct perspective of scientific communication compared to citations. They measure the cultural hole between two fields using trigrams and calculate the ratio of entropy within one field to the Kullback–Leibler divergence between both fields. They combine this language-based metric with citation distances to visualize a topological map of science. Our work differs from theirs in that we focus on the \textit{distinctiveness} of words or meanings, rather than distributional differences of phrases. \todo{add sentence about how our dataset is bigger.} In addition, we examine further as to why language and citations may provide different estimates of scientific proximity.

\section{Citation analysis}

Citation information continues to be the backbone of most science of science studies \cite{fortunato2018science}. To situate our paper against this broader focus, we examine the affordances of linguistic-based measures of scientific proximity compared to citation-based ones. That is, we highlight aspects of science that language-based measures emphasize more so than citation information does. The analyses in this section operate at the journal-level, so that each set of abstracts $s$ in NPMI calculations is a journal.

\todo{this may be moved} Citation-based measures of field or journal proximity have a few pitfalls, including the presence of non-connected components, missing citation information \cite{marx2015causes}, and a long tail of infrequently cited articles \cite{price1965networks}. In addition, every citation is treated as equal in the creation of these graphs, glossing over their multifaceted intentions and functions in an article \cite{teplitskiy2022status,prabhakaran-etal-2016-predicting,jurgens-etal-2018-measuring}. 

\subsection{Citation distance}

For a citation-based measure, we adopt \citet{vilhena2014finding}'s metric of \textit{citation distance}. \todo{define} Our citation graph does not subsample large journals. 

\subsection{Linguistic distances} 

We then calculate \textit{linguistic insularity} between journals, which is the correlation of their word and sense NPMI scores, and their \textit{linguistic gap}, which is the size of their non-overlap in positive NPMI words or senses. 

\subsection{Correlation \& disagreements}

We find that citation distance has a slight negative correlation with linguistic insularity, and a slight positive correlation with linguistic gap. This matches our intuition that language differences may present a barrier to citation-based communication between journals, a finding that matches the conclusion of previous work \cite{vilhena2014finding}.

\todo{not done yet.} We compare disagreements between citation distance and language-based measurements. This may help us create testable hypotheses on what factors may be involved in citation-based relatedness that are not in language-based relatedness, and vice versa. Possible factors: prestige, discipline, interdisciplinarity, sparsity of citation info (average citations per article), and highly cited methods e.g. statistics. We can also see if there are differences in the citation and language metric distributions of high-impact, ``general purpose'' journals versus other journals. An ideal, hard-hitting finding would be "citation distance may overestimate/underestimate disciplinary similarity due to the prestige and citation norms of a journal, but language is less affected". 

\subsection{Journal subject-area study}

\todo{not done yet.} We hypothesize that language can provide a more clear cut separation of journals' disciplines than citation distance. For example, the presence of high impact, high centrality articles (e.g. \textit{Nature} articles, articles for common statistical methods) may lead to underestimation of disciplinary distance between journals. Existing subject categorization schemes for journals use citation information (e.g. Web of Science, \citet{archambault2011towards}) or article text (e.g. MAG and S2 FOS) to assign journals to categories. To see how language compares to citation behavior when separating journal into disciplines, we need a ``gold'' discipline categorization scheme that does not use citations or article content. I propose experimenting with a subset of our dataset where disciplines are defined as journals whose titles share salient keywords, e.g. \textit{Pediatr-}. We can compare the following approaches: citation distance, word type alone, type + sense together. In what groups of journals are the biggest gains for separability and cohesiveness if we include word senses? 

\subsection{Methods}

After labeling occurrences of each vocab word with their senses, we calculate a metric $M$ that measures the distinctiveness of a word sense to a field or journal/venue. That is, if a sense $t_i$ of word $t$ is specific to a domain $s$, then this metric $M$ should indicate that 

\begin{enumerate} 
\item $t_i$ is prominent in $s$, or $M(s, t_i)$ is relatively high.
\item $t_i$ differentiates $s$ from any other domain $r$. That is, $M(s, t_i) > M(r, t_i)$.
\end{enumerate}

NPMI, like in the case of word types, can be a useful candidate metric because it takes in account the probability of $t_i$ across all abstracts, as well as the probability of it occurring in the target domain $s$. This roughly fits the two criteria above. In \citet{lucy-bamman-2021-characterizing}, type NPMI and sense NPMI are the same formula, where the event space for probabilities is over the occurrences of all words in a dataset. That is, sense NPMI is the same as type NPMI, except rather than counting occurrences of word $t$, they count occurrences of one of its senses, e.g. $t_i$.

Thus, our formula uses a different event space, or denominator, from \citet{lucy-bamman-2021-characterizing}, to avoid a word's type NPMI inflating its sense NPMI scores. Our formula for sense NPMI of the $i$th sense of word $t$ in a set of abstracts $s$ is the following: 

$$\textrm{NPMI}^\ast_s(t_i) = \frac{\log{ (P^\ast(t_i \mid s) / P^\ast(t_i))}}{-\log{P^\ast(t_i, s)}}.$$ Here, $P^\ast$ is the probability of the $i$th sense occurring over all senses of $t$. We only calculate NPMI for senses that appear at least 20 times in $s$. \todo{Jesse I wrote down in my notes what you said but then realized it is a little bit vague so I will copy paste it here and then you can help make it less hand-wavey? Word sense NPMI and type NPMI no longer share the same event space, but they’re different in the same way so they have some comparability amongst each other, but we recognize that they will have a different interaction than the standard NPMI. The comparison of two different sense NPMI scores will have a different interpretation, but we have other goals we want to meet.}

==> titles_brainstorm.tex <==
scholarly Jargon Discovery via Word Type and Sense Induction

Words as Academia's Gatekeepers: Measurement of Scholars' Use of Specialized Words and Senses 
Words as Academia's Gatekeepers: Inductive Measurement of Scholars' Use of Specialized Words and Senses


Words as Gatekeepers: Specialized Language as 
Words as Gatekeepers: Specialized Terminology vs General Language use In Science


Words as Gatekeepers: Measuring [word for Jargon] in Scholarly Publications
Words as Gatekeepers: Measuring Specialized Language in Scholarly Publications

Words as Gatekeepers: Measuring Discipline-specific Words and Meanings in Scholarly Publications

Words as Gatekeepers: Measuring Discipline-specific Word Types and Meanings in Scholarly Publications

Words as Gatekeepers: Measuring Discipline-Specific Lexical Items and Senses in Scholarly Publications

Words as Gatekeepers: Inducing Discipline-Specific Type and Sense Lexicons from Scholarly Publications

Note: we already say "words" once in the first part so maybe not "words" again in the second part

Words as Gatekeepers: Measuring Discipline-specific Language in Scholarly Publications

Words as Gatekeepers: Measuring Discipline-specific Terminology in Scholarly Publications

Words as Gatekeepers: Discipline-specific Language in Scholarly Publications and Their Implications

Here are some generated by ChatGPT:
"Deciphering Scholarly Jargon: A Computational Approach"
"Discipline-Specific Language in Scholarly Texts: Implications for Science Communication"
"The Role of Jargon in Interdisciplinary Impact: A Quantitative Analysis"
"Examining the Use and Effect of Jargon in Scientific Writing"
"Overcoming the Barrier of Jargon in Scientific Communication"
"Computational Approaches to Analyzing Discipline-Specific Jargon in Scholarly Text"
"Using Word Sense Induction to Characterize Scholarly Jargon Across Disciplines"
"Language as a Bridge or Barrier: A Computational Analysis of Jargon in Scientific Communication"
"Computational Sociolinguistics and the Science of Science: Examining the Use and Impact of Jargon"
"Computationally-Informed Insights into the Role of Jargon in Interdisciplinary Communication"


I like "Language as a Bridge or Barrier" lol
